CCSI: Continual Class-Specific Impression for Data-free Class Incremental Learning

In real-world clinical settings, traditional deep learning-based classification methods struggle with diagnosing newly introduced disease types because they require samples from all disease classes for offline training. Class incremental learning offers a promising solution by adapting a deep network trained on specific disease classes to handle new diseases. However, catastrophic forgetting occurs, decreasing the performance of earlier classes when adapting the model to new data. Prior proposed methodologies to overcome this require perpetual storage of previous samples, posing potential practical concerns regarding privacy and storage regulations in healthcare. To this end, we propose a novel data-free class incremental learning framework that utilizes data synthesis on learned classes instead of data storage from previous classes. Our key contributions include acquiring synthetic data known as Continual Class-Specific Impression (CCSI) for previously inaccessible trained classes and presenting a methodology to effectively utilize this data for updating networks when introducing new classes. We obtain CCSI by employing data inversion over gradients of the trained classification model on previous classes starting from the mean image of each class inspired by common landmarks shared among medical images and utilizing continual normalization layers statistics as a regularizer in this pixel-wise optimization process. Subsequently, we update the network by combining the synthesized data with new class data and incorporate several losses, including an intra-domain contrastive loss to generalize the deep network trained on the synthesized data to real data, a margin loss to increase separation among previous classes and new ones, and a cosine-normalized cross-entropy loss to alleviate the adverse effects of imbalanced distributions in training data.

==> sections/biography.tex <==
\section{Authotr Biography}

\noindent\textbf{Sana Ayromlou}

Sana Ayromlou is a Master's student in the Universit of British Columbia. She recieved her BSc (2021) from Sharif University of Technology, Iran. Her research interest is applying deep learning methods on more realistic scenarios in healthcare such as continual leaning and federated learning.


\noindent\textbf{Tresa Tsang}

Tresa Tsang is a cardiologist, Director of Echocardiography at Vancouver General Hospital and UBC Hospital, and Professor of Medicine,  Associate Head of Research for the Department of Medicine. In January 2017, Dr. Tsang was appointed Co-Acting Head for UBC Department of Medicine.
Dr. Tsang completed medical school at the University of Alberta and proceeded to Internal Medicine and Cardiology Fellowships at the U of A.  During her cardiology fellowship she was awarded both Medical Research Council of Canada and Alberta Heritage Foundation for Medical Research awards, under which she studied Clinical Epidemiology at the National Institutes of Health in Bethesda, Maryland.  After a year as staff cardiologist at Vernon Jubilee Hospital in B.C., Dr. Tsang began a Fellowship in Echocardiography at the Mayo Clinic, Rochester, Minnesota.   She was subsequently offered a staff position in Cardiology at Mayo Clinic, where she worked for more than 10 years as a clinician and researcher.   During this period, she was appointed Associate Professor of Medicine, and Consultant in Cardiology (2002), and subsequently Professor of Medicine (2006).  

Dr. Tsang’s research program is principally focused on physiologic and pathophysiologic aging of the cardiovascular system, and the prediction and prevention of adverse age-related cardiovascular events, including atrial fibrillation heart failure, stroke, and cognitive dysfunction. Her team has been investigating the use of advanced echocardiographic techniques to detect changes in the structure or function of individual heart chambers, and how these changes are associated with future development of disease.

\noindent\textbf{Purang Abolmaesumi}

Purang Abolmaesumi received his BSc (1995) and MSc (1997) from Sharif University of Technology, Iran, and his PhD (2002) from UBC, all in electrical engineering. From 2002 to 2009, he was a faculty member with the School of Computing, Queen’s University. He then joined the Department of Electrical and Computer Engineering at UBC, where he is a Canada Research Chair, Tier II, in Biomedical Engineering and a Professor, with Associate Membership to the Department of Urologic Sciences. He is also the recipient of the Killam Faculty Research Prize and the Killam Award for Excellence in Mentoring at UBC. 

Dr. Abolmaesumi is internationally recognized and has received numerous awards for his pioneering developments in medical image analysis and image-guided interventions. Dr. Abolmaesumi carries out research in medical imaging, machine learning, and image-guided diagnosis and interventions. Artificial intelligence and machine learning techniques are applied to diagnosis in ultrasound, magnetic resonance imaging, digitized pathology slides and other tissue images.

\noindent\textbf{Xiaoxiao Li}

Xiaoxiao Li is an Assistant Professor in the Electrical and Computer Engineering Department at the University of British Columbia (UBC). Before joining UBC, Dr. Li was a Postdoc Research Fellow in the Computer Science Department at Princeton University. Dr. Li obtained her PhD degree from Yale University in 2020. Dr. Li received her bachelor’s degree from Zhejiang University in 2015. In the recent few years，Dr. Li has over 30 papers published in leading machine learning conferences and journals, including NeurIPS, ICML, ICLR, MICCAI, IPMI, BMVC, AAAI, and Medical Image Analysis. Her work has been recognized with the OHBM Merit Abstract Award, the MLMI Best Paper Award, and the DART Best Paper Award. In addition, she has received travel awards from NeurIPS/ICML/MICCAI/IPMI. Dr. Li has also organized a number of workshops on the topic of machine learning and healthcare. She is the Associate Editor of Frontiers in NeuroImaging and a reviewer for a number of international conferences and journals.

Dr. Li’s research interests range across the interdisciplinary fields of deep learning and biomedical data analysis, aiming to improve the trustworthiness of AI systems for healthcare.
